SVD-LLM V2: Optimizing Singular Value Truncation for Large Language Model Compression

Despite significant advancements, the practical deployment of Large Language Models (LLMs) is often hampered by their immense sizes, highlighting the need for effective compression techniques. Singular Value Decomposition (SVD) is a promising LLM compression technique. However, existing SVD-based compression methods fall short in reducing truncation losses, leading to less competitive performance in compressed models. In this work, we introduce SVD-LLM V2, a SVD-based LLM compression method that optimizes singular value truncation in SVD compression with two techniques. First, SVD-LLM V2 proposes to use theoretical truncation loss of weight matrices to assign a unique compression ratio to each weight matrix at different layers to accommodate weight redundancy heterogeneity. Second, SVD-LLM V2 proposes loss-optimized weight truncation to ensure that the truncated singular values result in a lower and more stable truncation loss in practice. We evaluate SVD-LLM V2 on ten datasets and five LLMs at various scales. Our results show SVD-LLM V2 outperforms state-of-the-art SVD-based LLM compression methods. Our code is available at https://github.com/AIoT-MLSys-Lab/SVD-LLM

==> proof.tex <==
\section{Noise-Enhanced SVD Truncation}
We add a noise {\small$\Delta W$} to the original weight matrix {\small$W$} and choose to compress {\small$W_n = W + \Delta W$} instead of {\small$W$}. Below we provide the proof that this modification greatly reduces the compression loss.

\vspace{-2mm}
{\small
\begin{equation}
\begin{split}
     L&=\left\|W X-W^{\prime} X\right\|_F\\
    &=\left\|W S S^{-1} X-\operatorname{SVD}(W_n S) S^{-1} X\right\|_F\\
    &=\left\|(W S-\operatorname{SVD}(W_n S)) S^{-1} X\right\|_F\\
    &=\left\|(W_n S -\Delta W S-\operatorname{SVD}(W_n S)) S^{-1} X\right\|_F\\
    &=\left\|(W_n S -\operatorname{SVD}(W_n S)) S^{-1} X - \Delta WX\right\|_F\\
    &=\left\|(W_n S -\operatorname{SVD}(W_n S)) S^{-1} X - \Delta WX\right\|_F\\
\end{split}
\label{formula:loss}
\end{equation}
}

\noindent Same as SVD-LLM, we constructs the whitening matrix {\small$S$}, which satisfies {\small$SS^T = XX^T$}. We then perform the SVD compression on {\small$W_nS$}. Therefore, the compression loss {\small$L$} is calculated based on Equation~\ref{formula:loss}.

\noindent Therefore, the upper-bound of the loss $L$ is:

\vspace{-2mm}
{\small
\begin{equation}
\begin{split}
     L \leq \left\|(W_n S -\text{SVD}(W_n S)) S^{-1} X\right\|_F + \left\|\Delta WX\right\|_F\\
\end{split}
\label{formula:deduct}
\end{equation}
}

\noindent We set {\small $\Delta W = \epsilon \times Q\times L$} , where {\small $L$} is obtained by the Cholesky decomposition of {\small $(XX^T)^{-1}$}, i.e. {\small$(XX^T)^{-1} = L^TL$ }, {\small $Q$} is the positive definite matrix and $\epsilon$ is a minimum value. We could get:

\vspace{-2mm}
{\small 
\begin{equation}
\begin{split}
     \left\|\Delta WX\right\|_F 
     &= \sqrt{\operatorname{trace}[(\Delta WX)^T \Delta WX]}\\
     &= \sqrt{\operatorname{trace}[\Delta WX(\Delta WX)^T ]}\\
     &= \sqrt{\operatorname{trace}[\Delta W XX^T \Delta W ^T]} \\
     &= \sqrt{\operatorname{trace}[\epsilon^2 QL(XX^T)L^TQ^T]} \\
     &= \sqrt{\operatorname{trace}[\epsilon^2 QL(L^TL)^{-1}L^TQ^T]} \\
     &= \sqrt{\operatorname{trace}[\epsilon^2 QLL^{-1}(L^T)^{-1}L^TQ^T]} \\
     &= \sqrt{\operatorname{trace}[\epsilon^2 QQ^T]} = \sqrt{\operatorname{trace}[\epsilon^2]} = \epsilon \approx 0 
\end{split}
\label{formula:d2}
\end{equation}
}

Therefore, the loss $L$ is about the same as {\small$\left\|(W_n S -\text{SVD}(W_n S)) S^{-1} X\right\|_F$} and is still about equal to the singular values of $W_n S$.

Therefore, our job is to design $Q$ to lower the singular values of $W_n S = (W-\Delta W)S$ and the target could be transformed into the minimization of the kernel function of $(W-\Delta W)S = WS - \epsilon \times Q LS$, as shown in Equation~\ref{formula:goal}, which could be resolved by ADMM algorithm.

\vspace{-2mm}
{\small
\begin{equation}
\begin{split}
     Q = \min_{Q} \left\|WS - \epsilon Q L S\right\|_*
\end{split}
\label{formula:goal}
\end{equation}
}

